Representative Feature Extraction During Diffusion Process for Sketch Extraction with One Example

We introduce DiffSketch, a method for generating a variety of stylized sketches from images. Our approach focuses on selecting representative features from the rich semantics of deep features within a pretrained diffusion model. This novel sketch generation method can be trained with one manual drawing. Furthermore, efficient sketch extraction is ensured by distilling a trained generator into a streamlined extractor. We select denoising diffusion features through analysis and integrate these selected features with VAE features to produce sketches. Additionally, we propose a sampling scheme for training models using a conditional generative approach. Through a series of comparisons, we verify that distilled DiffSketch not only outperforms existing state-of-the-art sketch extraction methods but also surpasses diffusion-based stylization methods in the task of extracting sketches.

==> figtex/01_teaser.tex <==
\begin{figure*}
  \includegraphics[width=1\linewidth]{figures/teaser.png}
  \caption{Results of Diffsketch.}
   \label{fig:teaser}
\end{figure*}

==> figtex/XC1_vae2.tex <==
\begin{figure*}[htb]
  \centering
  \includegraphics[width=\linewidth]{figures/supp_vae2_vert.PNG}
  \vspace{-3mm}
  \caption{Extended Visualization of features from UNet and VAE.}

   \label{fig:sup_vae2}
\end{figure*}

==> figtex/XE2_qualitative3.tex <==
\begin{figure*}[htb]
  \centering
  \includegraphics[width=1\linewidth]{figures/added.png}
  %\vspace{-1.0em}
  \caption{Additional results of DiffSketch and $\text{DiffSKetch}_{distilled}$.}
   \label{fig:additionalvis}
\end{figure*}
